Online Service Caching and Routing at the Edge with Unknown Arrivals

This paper studies a problem of jointly optimizing two important operations in mobile edge computing without knowing future requests, namely service caching, which determines which services to be hosted at the edge, and service routing, which determines which requests to be processed locally at the edge. We aim to address several practical challenges, including limited storage and computation capacities of edge servers and unknown future request arrival patterns. To this end, we formulate the problem as an online optimization problem, in which the objective function includes costs of forwarding requests, processing requests, and reconfiguring edge servers. By leveraging a natural timescale separation between service routing and service caching, namely, the former happens faster than the latter, we propose an online two-stage algorithm and its randomized variant. Both algorithms have low complexity, and our fractional solution achieves sublinear regret. Simulation results show that our algorithms significantly outperform other state-of-the-art online policies.

==> sections/online_algorithm.tex <==
\section{Online Algorithm}
\label{sec:algorithm}

In this section, we present a two-stage online algorithm that jointly optimizes the service caching and routing problems. After arrival rates are revealed in each time slot, the first stage optimizes the routing decisions and produces necessary parameters for the next stage. Then, the second stage updates caching decisions for the next time slot.

\subsection{Optimal routing and subgradient at $X_t$}

We first consider the service routing problem, which entails finding $Y_t$ after $X_t$ is fixed and $\Lambda_t$ is observed. Without loss of generality, we assume that $d_1\geq d_2\geq\dots\geq d_N$.

Since $X_t$ and $\Lambda_t$ are known, finding the optimal $Y_t$ is equivalent to solving the following standard convex optimization problem:
\vspace{-2mm}
\begin{align}
    G_t(X_t):=\min_{Y_t} \quad& L_t(Y_t), \label{eq:rout_obj}\\
    \textrm{s.t.} \quad& y_{n,t}\leq x_{n,t}, \quad \forall n, \label{eq:rout_cons1}\\
    & 0\leq y_{n,t}, \quad \forall n. \label{eq:rout_cons2}
\end{align}

Solving (\ref{eq:rout_obj}) -- (\ref{eq:rout_cons2}) with standard convex optimization solvers may incur high complexity. Surprisingly, we show that there exists an $O(N)$ algorithm that not only solves (\ref{eq:rout_obj}) -- (\ref{eq:rout_cons2}) but also finds $\nabla G_t(X_t)$, which is required for calculating $X_{t+1}$.

The main idea of our algorithm is to leverage the special structure in $L_t(Y_t)$. Let 
\begin{align*}
    J_t(Y_t) := C(\sum_{n=1}^{N}\lambda_{n,t}y_{n,t})+\sum_{n=1}^{N}\lambda_{n,t}y_{n,t} C^{'}(\sum_{m=1}^{N}\lambda_{m,t}y_{m,t}).
\end{align*}
Then, $\frac{\partial L_t(Y_t)}{\partial y_{n,t}} = \lambda_{n,t}(J_t(Y_t) -d_n)$, which corresponds to the marginal benefit of processing one more request for service $n$ at the edge, is decreasing in $n$. Based on this observation, we design Alg.~\ref{alg:routing}.

\begin{algorithm}   
\caption{ServiceRouting} 
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\REQUIRE $d_1 \ge  d_2 \ge \ldots \ge d_N$, $X_t, \Lambda_t$
\renewcommand{\algorithmicrequire}{\textbf{Initialize:}}
\REQUIRE $Y_t\leftarrow 0$
\FOR{$n=1,2,...,N$}
\IF{$J_t(Y_t)-d_n<0$}
\STATE $y_{n,t}\leftarrow x_{n,t}$
\IF{$J_t(Y_t)-d_n>0$}
\STATE choose $y_{n,t}$ so that $J_t(Y_t)-d_n=0$
\ENDIF
\ENDIF
\ENDFOR
\FOR{$n=1,2,...,N$}
\IF{$J_t(Y_t) \leq d_n$}
\STATE $\nu_n\leftarrow \lambda_{n,t}(d_n-J_t(Y_t))$, $\mu_n\leftarrow 0$
\ELSE
\STATE $\nu_n\leftarrow 0$, $\mu_n\leftarrow \lambda_{n,t}(J_t(Y_t)-d_n)$
\ENDIF
\ENDFOR
\renewcommand{\algorithmicrequire}{\textbf{Output:}}
\REQUIRE $Y_t, \nabla G_t(X_t) \leftarrow [-\nu_1, -\nu_2,\dots,-\nu_N]$
\end{algorithmic}
\label{alg:routing}
\end{algorithm}
\vspace{-2mm}

\begin{theorem}
    Alg.~\ref{alg:routing} produces the optimal solution for the problem (\ref{eq:rout_obj}) -- (\ref{eq:rout_cons2}) and obtains the subgradient $\nabla G_t(X_t)$ 
\end{theorem}
\begin{IEEEproof}
    Let $Y_t^*$ be the solution produced by Alg.~\ref{alg:routing}. We first prove that $Y_t^*$ is optimal by using KKT conditions.
    
    Let $\nu_n$ and $\mu_n$ be Lagrange multipliers associated with (\ref{eq:rout_cons1}) and (\ref{eq:rout_cons2}), respectively. KKT conditions for (\ref{eq:rout_obj}) -- (\ref{eq:rout_cons2}) are
    \begin{align}
        \lambda_{n,t}(J_t(Y_t) - d_n) - \mu_n + \nu_n = 0, \forall n, \label{eq:KKT1} \\
        \nu_n (y_{n,t} - x_{n,t})=0, \mu_{n}(-y_{n,t}) = 0, \forall n, \label{eq:KKT2}\\
        \mu_n \geq 0,\; \nu_n \geq 0, \forall n. \label{eq:KKT3}
    \end{align}
    
    It is obvious that $Y_t^*$ satisfies conditions (\ref{eq:KKT1}) and (\ref{eq:KKT3}). Thus, we only need to show that it also satisfies the condition (\ref{eq:KKT2}). In particular, we need to prove following two claims: If $y_{n,t}^*=x_{n,t}>0$, then $J_t(Y_t^*)\leq d_n$. If $y_{n,t}^*=0$ and $x_{n,t}>0$, then $J_t(Y_t^*)\geq d_n$.
    
    Let $m^*$ be the last service with $y_{m^*,t}^*>0$. When $y_{n,t}>0$, we have $m^*\geq n$ and hence $d_{m^*}\leq d_n$. By the design of Steps 1 -- 5 in Alg.~\ref{alg:routing}, $J_t(Y_t)^*\leq d_{m^*}\leq d_n$. When $y_{n,t}^*=0$ and $x_{n,t}>0$, we have $J_t(Y_t^*)\geq d_n$ by the end of the $n$-th iteration of the first for loop. Since $Y_t^*$ can only be increased in latter iterations and $J_t(Y_t^*)$ is an increasing function, we have $J_t(Y_t^*)\geq d_n$. Therefore, both claims are proved.
    
    %Consider the case $y_{n,t}^*=x_{n,t}>0$. Let $m^*$ be the last service that chooses $y_{m^*,t}^*>0$. Since $y_{n,t}^*>0$, we have $m^*\geq n$ and hence $d_{m^*}\leq d_n$. By the design of Steps 1 -- 5 in Alg.~\ref{alg:routing}, we have $J_t(Y_t)^*\leq d_{m^*}\leq d_n$ when Steps 1 -- 5 are completed. This proves the first claim.
    
    %Next, we consider the case $y_{n,t}^*=0$ and $x_{n,t}>0$. By the design of Steps 1 -- 5 in Alg.~\ref{alg:routing}, we have $J_t(Y_t^*)\geq d_n$ by the end of the $n$-th iteration of the for loop. Since $Y_t^*$ can only be increased in latter iterations and $J_t(Y_t^*)$ is an increasing function, we have $J_t(Y_t^*)\geq d_n$ when Steps 1 -- 5 are completed. This proves the second claim.
    
    Then, we prove Alg.~\ref{alg:routing} provides the subgradient $\nabla G_t(X_t)$.
    
    It can be shown that $G_t(X_t)$ is convex. Then, based on \cite[\S 5.6]{Boyd2004Conv}, we have
    \begin{equation}
        \frac{\partial G_t(X_t)}{\partial x_{n,t}}  = -  \nu_n  = 
        \begin{cases}
            &  \lambda_{n,t}(J_t(Y_t^{*})-d_n), \textbf{ if } y_{n,t}^{*} = x_{n,t}, \\
            & 0, \qquad\qquad\qquad\quad\; \textbf{otherwise},
        \end{cases}
        \nonumber
    \end{equation}
    and $\nabla G_t(X_t) = [\frac{\partial G_t(X_t)}{\partial x_{1,t}},\dots,\frac{\partial G_t(X_t)}{\partial x_{N,t}}]$.
\end{IEEEproof}

Furthermore, we have the following corollary.
\begin{corollary}
    The subgradient $\nabla G_t(X_t)$ is bounded by $\| \nabla G_t(X_t)\|_2^{2} \leq W^{2}d_{1}^{2}$.
    \label{corro:bound}
\end{corollary}
\begin{IEEEproof}
    As $d_n$s are sorted in descending order, we have $\|\nabla G_t(X_t)\|_2^2 = \sum_{n=1}^{N} \nu_n^2 \leq \sum_{n=1}^{N} \lambda_{n,t}^2 d_n^2 \leq W^2 d_1^2.$
\end{IEEEproof}

\subsection{Online caching updates and OCR algorithm}

We consider the following Alg.~\ref{alg:caching} for the online service caching update, which is mainly adopted online gradient descent with lazy projection in \cite{Shai2012OCO}. In Alg.~\ref{alg:caching}, $\nabla G_t(X_t)$ is the subgradient of the function $G_t(X_t)$ calculated by Alg.~\ref{alg:routing}, $\eta$ is the step size, and $\theta_t=[\theta_{1,t},\theta_{2,t},\dots,\theta_{N,t}]$ is an internal vector with $\theta_1=\textbf{0}$.
\vspace{-1mm}
\begin{algorithm}   
\caption{ServiceCaching} 
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\REQUIRE $\theta_{t},\nabla G_{t}(X_{t}),\eta$
\STATE $\theta_{t+1}=\theta_{t}-\nabla G_{t}(X_{t})$
\STATE $X_{t+1} \leftarrow$ the Euclidean projection of $\eta\theta_{t+1}$ onto the set $\{X\in \mathbb{R}^N~|~0\leq x_{n}\leq 1, \; \sum_{n=1}^{N}x_{n}\leq Z\}$
\renewcommand{\algorithmicrequire}{\textbf{Output:}}
\REQUIRE $X_{t+1},\theta_{t+1}$
\end{algorithmic}
\label{alg:caching}
\end{algorithm}
\vspace{-2mm}

In each time slot, Alg.~\ref{alg:caching} updates the internal variable $\theta_t$ by $\theta_{t+1}=\theta_{t}-\nabla G_{t}(X_{t})$, and then calculates the caching decision $X_{t+1}$ by projecting $\eta\theta_{t+1}$ onto the domain of $X_t$.
\vspace{-1mm}
\begin{algorithm}
\caption{Online service Caching and Routing (OCR)}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Initialize:}}
\REQUIRE $\eta$, $\theta_1\leftarrow 0$, $X_1$
\FOR{$t=1,2,...,T$}
\STATE $Y_t, \nabla G_t(X_t)\leftarrow ServiceRouting(X_t,\Lambda_t)$
\STATE $X_{t+1},\theta_{t+1} \leftarrow ServiceCaching(\theta_{t},\nabla G_{t}(X_{t}),\eta)$
\ENDFOR
\end{algorithmic}
\label{alg:OCR}
\end{algorithm}
\vspace{-2mm}

Then, our online service caching and routing algorithm (OCR) is shown as Alg~\ref{alg:OCR} with following results.

\begin{theorem}
    By choosing $\eta=O(\frac{1}{\sqrt{T}})$, the regret of applying OCR is $Reg(OCR)=O(\sqrt{T})$.
\end{theorem}
\begin{IEEEproof}
    It is easy to verify that $\beta \|X_t-X_{t-1}\|_+ \leq \beta \|X_t-X_{t-1}\|_1$. Thus, the regret of OCR is upper bounded by the regret of applying online gradient descent with lazy projection on $\sum_{t=1}^{T}(G_t(X_t)+\beta \|X_t-X_{t-1}\|_1 )$.
    
    By choosing $\eta=O(\frac{1}{\sqrt{T}})$, Corollary 2.17 in \cite{Shai2012OCO} shows that the regret of online gradient descent with lazy projection on objective $G_t(X_t)$ with bounded subgradient is $O(\sqrt{T})$. Then, based on Corollary 1 in \cite{lin2012online}, the regret is still $O(\sqrt{T})$ after introducing one-norm term $\beta \|X_t-X_{t-1}\|_1$.
    
    Therefore, the regret of applying OCR is $Reg(OCR)=O(\sqrt{T})$ when $\eta=O(\frac{1}{\sqrt{T}})$.
\end{IEEEproof}

Finally, we analyze the complexity of Alg.~\ref{alg:OCR}. It can be verified that the bottleneck is the projection step in the line 2 of Alg.~\ref{alg:caching}, which can be solved in $O(N^2)$ by using the projection algorithm mentioned in Paschos \emph{et al.} \cite{paschos2019learning}. Hence, the overall complexity of Alg. 3 is $O(N^2)$ per time slot.

%We consider the following steps for the projection. Let $X'$ be the vector where $x'_n = \min\{1,\max\{0,\eta \theta_{n,t}\}\}$. If $\sum_{n=1}^N x'_n\leq Z$, then $X'$ is the projection. Otherwise, the projection, denoted by $X^*$, must have $\sum_{n=1}^N x^*_n=Z$. Then, we can employ the algorithm in \cite{wang2015projection}, which has complexity $O(N^2)$, to obtain $X^*$. 



==> sections/system_model.tex <==
\section{System Model}
\label{section:model}

\subsection{System Overview}

We consider an edge system with a backhaul connection. This edge system includes multiple clients, an edge server, and remote data centers. Clients generate requests for different services according to some unknown and unpredictable patterns, and then send these requests to the edge server. We use $N$ to denote the total number of different services. The edge server may \emph{cache} some services and process some requests for these services locally, while forwarding remaining requests to remote data centers. Requests processed at the edge encounter a \emph{computation latency} due to the limited computation capacity of the edge server, while requests forwarded to remote data centers encounter a \emph{forwarding latency} due to network latencies.

\subsection{Service Caching and Processing}

We assume that time is slotted, and the system runs for $T$ time slots. The duration of a time slot is chosen so that, in any given time slot, the patterns for the service requests (originating from different clients) remain roughly the same.

Let $x_{n,t}\in\{1,0\}$ be a binary decision variable that indicates whether the edge server caches service $n$ in time slot $t$, and let $X_{t}:=[x_{1,t},x_{2,t},\dots,x_{N,t}]$. Since the edge server has limited storage capacity, we assume that the edge server can cache at most $Z$ services, i.e., $\sum_{n=1}^{N} x_{n,t}\leq Z,\forall t$. We call the problem of determining $X_t$ the \emph{service caching problem}. 

Caching a new service at the edge can be a costly process, which typically involves downloading codes and databases and setting up virtual machines or containers. Thus, we assume that the edge server must decide $X_t$ before time slot $t$.

At the beginning of time slot $t$, the edge server observes the requests from clients and calculates the request arrival rates. We use $\lambda_{n,t}$ to denote the number of requests for service $n$ in time slot $t$, and let $\Lambda_t:=[\lambda_{1,t},\lambda_{2,t},\dots,\lambda_{N,t}]$. We assume that an upper bound $W$ on the total arrival rate is known, that is, $\sum_{n=1}^{N}\lambda_{n,t}\leq W,\forall t$.

%During each time slot $t$, the edge server needs to decide which requests to be processed locally. Due to the limited computation power, the edge server processes $y_{n,t}$ requests for the service $n$, and forwards the remaining $(\lambda_{n,t}-y_{n,t})$ requests to remote data centers. Since the edge server can only process requests whose corresponding services have already been cached at the edge, we require that $y_{n,t}\leq \lambda_{n,t}x_{n,t}$.

During each time slot $t$, the edge server needs to decide which requests to be processed locally. Due to the limited computation power of the edge server, it may not be desirable to process all requests for services that it caches. For a service $n$, the edge server will process a fraction $y_{n,t}$ of the requests locally, and forward the remaining $(1-y_{n,t})$ portion of the requests to the data center. Since the edge server can only process requests whose corresponding services have already been cached at the edge, we require that $y_{n,t}\leq x_{n,t}, \forall n$.


Let $Y_t:=[y_{1,t},y_{2,t},\dots,y_{N,t}]$.  %denotes the vector that collects all $y_{n,t}$. 
We call the problem of determining $Y_t$ the \emph{service routing problem}. Since the edge server can adjust service routing in real time, we consider that the edge server determines $Y_t$ after it observes $\Lambda_t$.

\subsection{Cost and Problem Formulation}

The goal of the edge server is to minimize the total cost of the system, which consists of \emph{installation cost} and \emph{latency cost}, by jointly optimizing $X_t$ and $Y_t$.

The installation cost refers to the operation cost incurred when the edge server caches new services. Since the total installation cost relates to the number of new services cached by the edge server, we assume that caching every new service incurs a cost of $\beta$. Hence, the total installation cost is $\beta \sum_{t=1}^{T}\|X_t-X_{t-1}\|_+$, where $\|X_t\|_+=\sum_{n=1}^{N}\max\{x_{n,t},0\}$.

The latency cost refers to the total latency experienced by all requests. In the system, when a request is forwarded to the remote data center, it experiences a forwarding latency, which is denoted as $d_{n}$ for service $n$. When a request is processed at the edge, it experiences a computation latency due to the limited computation power of the edge server. It is reasonable to assume that the per-request computation latency at the edge depends on the total computation load, and can be described by a convex, increasing, and differentiable function $C(\cdot)$ with $0 \le C(0) \leq d_n, \forall n$ and $\lim_{s\to\infty} C(s) = \infty$. Since the total computation load at the edge server is $\sum_{n=1}^{N}\lambda_{n,t}y_{n,t}$ in time slot $t$, the total latency of all requests can be written as
\begin{align*}
    L_t(Y_t) := \sum_{n=1}^{N} \lambda_{n,t}y_{n,t} C\big( \sum_{m=1}^{N}\lambda_{m,t}y_{m,t}\big) + \sum_{n=1}^{N} \lambda_{n,t}(1 - y_{n,t})d_n.
\end{align*}

As a result, the sequence of determining variables and receiving cost is summarized as Fig.~\ref{fig:processes}, and the total cost over $T$ time slots can be written as $\sum_{t=1}^{T}(L_t(Y_t)+\beta \|X_t-X_{t-1}\|_+)$.
\vspace{-4mm}
\begin{figure}[thpb]
    \centering
    \includegraphics[scale=0.18]{figures/Figure2.PNG}
    \caption{Process of online service caching and routing.}
    \label{fig:processes}
    \vspace{-2mm}
\end{figure}

The edge server aims to find $[X_1,X_2,\dots,X_T]$ and $[Y_1,Y_2,\dots,Y_T]$ that minimize the total cost. To make the optimization problem convex, we further relax the integer constraint on $x_{n,t}$ and allow $x_{n,t}$ to be any real number in $[0,1]$. Under the relaxation, $x_{n,t}$ can be interpreted as the probability of caching service $n$ at time $t$. After the relaxation, the (offline) problem of minimizing the total cost can be written as follows:
\begin{align}
    \min_{[X_t],[Y_t]} \quad & \sum_{t=1}^{T}\Big(L_t(Y_t)+\beta \|X_t-X_{t-1}\|_+ \Big), \label{equation:OCO_intro} \\
    \textrm{s.t.} \quad& 0\leq x_{n,t}\leq 1, \quad \forall n, \forall t, \\
    \quad& 0\leq y_{n,t} \leq x_{n,t}, \quad  \forall n, \forall t, \\
    & \sum_{n=1}^{N}x_{n,t}\leq Z, \quad  \forall t.
\end{align}

While the above problem is a standard convex optimization problem, solving it requires the knowledge of all request arrival rates, that is, all $\Lambda_t$, in advance. In practice, however, the edge server needs to make service caching and routing decisions, which are $X_t$ and $Y_t$, without the knowledge of future arrival rates. Moreover, as the process shown in Fig.~\ref{fig:processes}, the service caching problem and the service routing problem operate on different timescales. The edge server needs to decide $X_t$ in time slot $t-1$, without any knowledge about $\Lambda_t$. In contrast, the edge server can decide the value of $Y_t$ after observing the first few requests in time slot $t$ to estimate the arrival rate $\Lambda_t$. The algorithm for determining these routing and caching decisions is called an \emph{online algorithm}.

The performance of an online algorithm is evaluated by comparing it against an offline policy. We consider that the offline policy knows the overall popularity of a service $n$, $\sum_t \lambda_{n,t}$, but not individual $\lambda_{n,t}$. In this case, the optimal offline algorithm will cache the largest $\sum_t \lambda_{n,t}d_n$ in all slots. The assumption for this optimal static offline policy is widely used in caching literature, such as \cite{bhattacharjee2020fundamental}. We let $X^o:=[x^{o}_1, x^{o}_2, \dots, x^{o}_N]$ be the service caching decision of the optimal static offline policy. In each time slot $t$, after learning $\Lambda_{t}$, the offline policy will choose the optimal vector $Y_t^o$ with $y^o_{n,t}\leq x_n^o,\forall n$ that minimizes $L_t(Y_t^o)$. 

%Hence, the offline policy will simply cache the same $Z$ services with the largest $\sum_t \lambda_{n,t}d_n$ in all slots. 

Let $\hat{X}:=[\hat{X}_1,\hat{X}_2,\dots,\hat{X}_T]$ and $\hat{Y}:=[\hat{Y}_1,\hat{Y}_2,\dots,\hat{Y}_T]$ be solutions produced by an online algorithm $\xi$, then we define the regret of $\xi$ as the difference between its cost and the optimal static offline policy's cost:
\begin{equation*}
    Reg(\xi) := \sum_{t=1}^{T}\big(L_t(\hat{Y}_t) - L_t(Y_t^{o}) +\beta\|\hat{X}_t-\hat{X}_{t-1}\|_+\big).
    \vspace{-1mm}
\end{equation*}
It should be noticed that the optimal static offline policy does not change its caching decisions and hence it doesn't suffer installation costs.

The goal of this paper is to find an online algorithm with provably small regret under any sequence of arrival rates.
